The no boundary density matrix

We discuss a no-boundary proposal for a subregion of the universe. In the classical approximation, this density matrix involves finding a specific classical solution of the equations of motion with no boundary. Beyond the usual no boundary condition at early times, we also have another no boundary condition in the region we trace out. We can find the prescription by starting from the usual Hartle-Hawking proposal for the wavefunction on a full slice and tracing out the unobserved region in the classical approximation. We discuss some specific subregions and compute the corresponding solutions. These geometries lead to phenomenologically unacceptable probabilities, as expected. We also discuss how the usual Coleman de Luccia bubble solutions can be interpreted as a possible no boundary contribution to the density matrix of the universe. These geometries lead to local (but not global) maxima of the probability that are phenomenologically acceptable.

==> ActFixedCurv.tex <==


If the integral over the manifold in the action for the problem in \nref{FixCurv} was over the whole sphere times a $\tau$ interval and all $\hat{c}_{l}$ were real then the action would reduce to \nref{OnshellactHH+Curv} computed before. However, the integration range is not of this form for every $\tau$, as shown in the diagram below (ADD DIAGRAM), and the $\hat{c}_{l}$ have imaginary parts.

Here I will try to clean up more the dicussion of the large time action. The point is to solve the equation of motion at large times. The equation for $\varphi$ is
\begin{equation}
\frac{1}{\cosh^{3}\tau}\partial_{\tau}((\cosh \tau)^{3}\partial_{\tau}\varphi)-\frac{1}{\cosh^{2}\tau}\nabla_{S^{3}}^{2}\varphi+3=0
\end{equation}

Taking the imaginary part of the equation of motion imply that the imaginary part of $\varphi$ satisfy the homogeneous equation of motion, so at large times it can be expanded as
\begin{equation}
\varphi^{+}-\varphi^{-}=g(\Omega_{3})e^{-3\tau_{0}}(1+O(e^{-2 \tau}))+h(\Omega_{3})e^{-3 \tau}(1+O(e^{-2 \tau}))
\end{equation}
where the subleading corrections all come from terms dependent on spatial derivatives of $g$ and $h$. Note that for consistency the prefactor of $g$ is of order $e^{-3\tau_{0}}$ so that it can cancel the $h$ term if $\vec{\Omega}_{3} \in \Sigma_{in}$ where the fields are real. Note that $h$ is determined from
\begin{equation}
\partial_{\tau}\varphi^{+}-\partial_{\tau}\varphi^{-}=-3 h(\Omega_{3})e^{-3 \tau}+...
\end{equation}
and $g$ is determined from requiring $\varphi^{+}-\varphi^{-}=0$ for $\vec{\Omega}_{3} \in \Sigma_{in}$ and $\tau=\tau_{0}+\rho$.
\begin{equation}
\varphi^{+}-\varphi^{-}=-\frac{1}{3}(\partial_{\tau}\varphi^{+}-\partial_{\tau}\varphi^{-})|_{\tau=\tau_{0}}(e^{-3(\tau-\tau_{0})}-e^{-3 \rho})\,.
\end{equation}

Note this works even if $\vec{\Omega}_{3} \in \Sigma_{out}$ because there we should have $\varphi^{+}=\varphi^{-}$ \VI{Will add point about vertical light cones before}. The action term coming from the Lorentzian section of the geometry at large $\tau$ is thus
\begin{equation}
\begin{gathered}
I_{L}\approx \frac{ \epsilon_{0}M_{pl}^{2}}{8 H_{0}^{2}}\int d\Omega_{3}\int_{0}^{\tau_{0}+\rho} d\tau (\partial_{\tau}\varphi^{+}-\partial_{\tau}\varphi^{-})|_{\tau=\tau_{0}}(e^{3\tau_{0}}-e^{3(\tau- \rho)})\\
\approx \frac{ \epsilon_{0}M_{pl}^{2}}{8 H_{0}^{2}}\int d\Omega_{3} (\partial_{\tau}\varphi^{+}-\partial_{\tau}\varphi^{-})|_{\tau=\tau_{0}}e^{3 \tau_{0}}(\tau_{0}+\rho)
\end{gathered}
\end{equation}
where we dropped terms of order $O(1)$ that do not depend on $\rho$. Note the coefficient of $\rho$ is exact since it comes from the large $\tau$ region of the integration range. Note the $\tau_{0}$ integral simplify since it is a integral of $\partial_{\tau}\varphi^{+}-\partial_{\tau}\varphi^{-}$ over $\Omega_{3}$. This projects to the singlet component of this discontinuity, which only comes from the inhomogeneous term $\varphi_{c}$, therefore giving
\begin{equation}
I_{L}\approx \frac{8 \pi^{2}i \epsilon_{0} M_{pl}^{2}}{H_{0}^{2}}\bigg(\tau_{0}-\frac{i}{64 \pi^{2}}\int d\Omega_{3} \rho\, e^{3 \tau_{0}}(\partial_{\tau}\varphi^{+}-\partial_{\tau}\varphi^{-})|_{\tau=\tau_{0}}\bigg)
\end{equation}

The contribution for the probability density from the euclidean part of the geometry is additive on the bra and ket, and thus comes only from the real part of $\varphi$. Since the integration is over the whole of $\Omega_{3}$, only the singlet component of $\varphi$ contribute, which is approximately constant, and the action is at leading order
\begin{equation}
I_{E} \approx -\frac{3 \epsilon_{0}M_{pl}^{2}}{H_{0}^{2}}\bigg(-i\frac{8 \pi^{2}}{3}\bigg)\bigg(c_{0}+\tau_{r}\bigg)=\frac{8 \pi^{2}i \epsilon_{0}M_{pl}^{2}}{H_{0}^{2}}(c_{0}+\tau)
\end{equation}
the total probability density is therefore
\begin{equation}
i I \approx \frac{8 \pi^{2}i \epsilon_{0}M_{pl}^{2}}{H_{0}^{2}}\bigg(2\tau_{0}+c_{0}-\frac{i}{64 \pi^{2}}\int_{\Sigma_{in}} d\Omega_{3} \rho\, e^{3 \tau_{0}}(\partial_{\tau}\varphi^{+}-\partial_{\tau}\varphi^{-})|_{\tau=\tau_{0}}\bigg)
\end{equation}

The strategy to compute the on-shell action is then to sum and subtract the integral of the scalar on-shell lagrangian in the region $S$, since the integral of the action including $S$ is of the form \nref{OnshellactHH+Curv}, plus an extra term coming from the imaginary part of $\tilde{c}_{0}$. The action in the problem under consideration is therefore
\begin{equation}
\begin{gathered}
i S=-\frac{8 \pi^{2}\epsilon_{0}M_{pl}^{2}}{H_{r}^{2}}\bigg(2 \tau_{0}-4 \ln 2+\frac{17}{6}+c_{0}+\frac{i e^{3 \tau_{0}}}{64 \pi^{2}}\int_{\Omega_{3}}(\tilde{\varphi}^{+}-\tilde{\varphi}^{-}) -\frac{3 i}{8 \pi^{2}}\int_{S}(\varphi^{+}-\varphi^{-})\bigg)
\end{gathered}
\end{equation}
with 

==> ComplexSols.tex <==
\VI{Here we want to explain well Juan's argument that for a solution to be at the maxima of probability it has to be real, this follows from for example relating the momenta of the field with the operator $\frac{\delta}{ \delta \phi}$.}

==> Cutouts.tex <==
 \subsection{More detailed prescription for the geometries}

Here we explain in more detail the boundary conditions that we are imposing. In particular, we will center on the so called ``trace-out'' boundary conditions for the region we do not observe. We can start from a full Cauchy slice for the full spacetime and then impose these conditions outside the $\Sigma_\pm$ regions. 
Let us call $\Sigma_{out}$ the region of the Cauchy slice that describes the region of the spacetime that we are tracing out, see figure \ref{SigmaInOut}.  
We impose the conditions 
\be \la{TrOut}
\Phi^+(x) = \Phi^-(x) ~,~~~~~~~\dot \Phi^+(x) = \dot \Phi^-(x)  ~,~~~~~~~{\rm for  } ~~~x \in \Sigma_{out}
\ee 
where $\Phi$ collectively denotes all the fields in the theory, the inflaton, the metric, etc. 

Let us   explain the rationale for these boundary conditions \nref{TrOut}. For simplicity, let us consider a simple quantum mechanical non-relativistic theory in a pure state with wavefunction $\psi(x)$. 
The density matrix is 
\be 
\rho(x_-,x_+) = \psi^*(x_-) \psi(x_+) 
\ee 
If we are interested in the trace of the density matrix we should set $x_-=x_+$ and integrate over $x_+$. 
Now, if we are using the semiclassical approximation, then $\psi(x_+)=e^{iS_+},  ~\psi^* = e^{ - i S(x_-)}$, where the action is evaluated on a solution $x_\pm(t)$ which reaches $x_\pm(t) = x_\pm$ at, say, $t=0$. 
The condition $x_+=x_-$ that comes because we are considering the trace imposes that the two boundary values of $x_\pm(t)$ are equal. The fact that we are integrating over this boundary value implies, via the saddle point approximation 
\be 
\int d x e^{ i S_+(x) - i S_-(x) } ~,~~~~~~\to ~~~~~\partial_x (S_+ - S_-) =0 ~,~~~~~~\to ~~~p_+ = p_- 
\ee 
or $\dot x_+ = \dot x_-$. In other words, by find a solution which obeys $x_+ = x_-$ and 
$\dot x_+ = \dot x_-$ we can directly compute the semiclassical approximation to the density matrix \YC{(Do we want to present harmonic oscillator example of this in appendix? Like Juan's review also quickly showed this how it works for harmonic oscillator)}. If instead of having a single quantum mechanical degree of freedom we have a field theory, and we are only tracing out over a subregion of the spacetime, then the same reasoning leads to the boundary conditions \nref{TrOut}.  


 
Note that we can pick many different slices for $\Sigma_{out}$. In fact,  in the Lorentzian spacetime, the solution obeys 
\nref{TrOut} everywhere  in the whole domain of dependence of $\Sigma_{out}$. 
In particular, this means that   we can take $\Sigma_{out}$ to lie very close to the backwards light cone of the regions $\Sigma_{\pm}$. As we go into Euclidean time, the $+$ and $-$ solutions can become different, since the prescription that takes us to Euclidean time are different for these two regions. However, the fact that they are continuously connected is still true. 


In principle, we could have situations where we have a geometry that prepares the density matrix but we have no geometry that prepares the wavefunction on some global slice. 


We will see later some examples of cases where the global slice geometries are less convenient to describe the wavefunction, but we have not found a situation where there is no pure state that the system could have come from. SAY THIS BETTER. 

In gravity, we can truly focus on the part of the geometry that computes the density matrix without ever talking about the geometry in the region we do not observe. This seems to be an elegant aspect of the proposal, but we have not found a killer application for it. 
MAYBE THIS SHOULD GO INTO THE DISCUSSION SESSION. 




 
 
%\input{Introduction.tex}
   
\subsection{Relation to Hartle Hawking wavefunction}
%\YC{Hartle Hawking prescription for the density matrix} \label{sec:complex}

\input{ReltoHH.tex}

%\subsection{Complex solutions are not at the maxima of probability}
%\YC{Reality condition at maxima of the probability}}
%\label{ComplexSol}

%\input{ComplexSols.tex}

\subsection{Properties of the Schwinger Keldysh contour}
%\YC{Schwinger-Keldysh contour and geometry}}

\input{SK.tex}


\subsection{The density matrix for the Weyl factor \JM{I would also eliminate this one} \VI{I agree with this if we write something like \nref{OnshellactHH} somewhere else in the paper. This is a useful formula with the $\tau$ and $c$ dependence together that is useful to reference later}}


\VI{I rewrote this section with the perspective we are computing the density matrix of $\varphi$ in a 3-geometry at $\tau=\tau_{r}$}

To exemplify the setup from the previous section, consider a problem where one constructs the density matrix for the inflaton by specifying either Dirichlet or trace out boundary conditions in the entire $\tau=\tau_{r}$ slice in global coordinates. One only fixes $\varphi$ in the bra and ket sides in some section $\Sigma_{in}$ of the sphere to be some fixed fixed functions of the three geometry $\varphi_{b}^{\pm}(\Omega_{3})$, and the bra and the ket are glued in the rest of the $\tau=\tau_{r}$ sphere where one must impose 
$\dot{\phi}^{+}=\dot{\phi}^{-}$ and $\phi^{+}=\phi^{-}$.

This computation is by definition the density matrix of the inflaton in the $\Sigma_{in}$ slice at $\tau=\tau_{r}$, but via the argument raised in subsection \nref{dmsubregion} if $\tau_{r}>>1$ this can also be interpreted as the density matrix for the Weyl factor $\rho=\varphi_{b}(\Omega_{3})$ of the 3-geometry where $\varphi=0$. We take the latter perspective and refer to the fixed field profile as $\rho$ from now on. In this discussion we will further restrict to solutions with $\rho^{+}=\rho^{-}$, which represents the diagonal components of this density matrix.

%We again decompose $\varphi^{\pm}=\varphi_{c}^{\pm}+\tilde{\varphi}^{\pm}$, with $\varphi_{c}^{\pm}$ the inhomogeneous solutions \nref{phic} that vanishes at $\tau=\tau_{r}$ and $\tilde{\varphi}_{\pm}$ a homogeneous solution that will enforce the boundary conditions. In terms of this splitting, the boundary conditions for $\tilde{\varphi}^{\pm}$ at $\tau=\tau_{r}$ are
%\begin{equation}
%\begin{gathered}
%\tilde{\varphi}^{+}|_{\tau=\tau_{r}}=\tilde{\varphi}^{-}|_{\tau=\tau_{r}}=\rho(\Omega_{3}) \text{ for $\vec{\Omega}_{3}\in \Sigma_{in}$}\\ \partial_{\tau}\tilde{\varphi}^{+}|_{\tau=\tau_{r}}-\partial_{\tau}\tilde{\varphi}^{-}|_{\tau=\tau_{r}}=-(\partial_{\tau}\varphi_{c}^{+}|_{\tau=\tau_{r}}-\partial_{\tau}\varphi_{c}^{-}|_{\tau=\tau_{r}}) \text{ for } \vec{\Omega}_{3} \in \Sigma_{out}
%\end{gathered}
%\end{equation}
The boundary conditions can be stated a bit more concretely by decomposing $\tilde{\varphi}$ in angular momentum modes on the sphere as in \nref{homexp} but taking more general dependences on $S^{3}$
\begin{equation}
\tilde{\varphi}^{\pm}=\sum_{l=0}^{\infty}c_{l,m_{1},m_{2}}Y_{l,m_{1},m_{2}}(\Omega_{3}) \frac{f_{l}^{\pm}(\tau)}{f_{l}^{\pm}(\tau_{r})} 
\end{equation}
in terms of which the Dirichlet boundary conditions are the same as in \nref{masslesscond}, so we used that $c_{l,m_{1},m_{2}}^{\pm}$ will be real and equal. However, as mentioned in \nref{EqnsTo2} the trace-out boundary condition is slightly different because of the presence of the $\varphi_{c}$ term, so that the trace out boundary conditions is now expressed as
\begin{equation}
\label{vfpr}
\sum_{l=1}^{\infty} l(l+1)(l+2)c_{l,m^{a}}Y_{l,m^{a}}(\Omega_{3})=-2 \text{ for }\vec{\Omega}_{3} \in \Sigma_{out}
\end{equation}

And in terms of this decomposition the action \nref{ActForF} can be readily evaluated using the orthogonality of the harmonics to give

%To evaluate the action of the solution at leading order in $V'$ we use the result \nref{OnshellactHH} derived in the previous subsection to write
%\begin{equation}
%\begin{gathered}
%
%I=\frac{\epsilon_{0} M_{pl}^{2}}{H_{r}^{2}}\bigg(3\int_{-\frac{i \pi}{2}}^{\tau_{r}}d\tau \int_{S^{3}}d\Omega_{3}\cosh^{3}\tau\, \varphi^{-}-3\int_{\frac{i \pi}{2}}^{\tau_{r}}d\tau \int_{S^{3}} d\Omega_{3}\cosh^{3}\tau\, \varphi^{+}\\
%+\int_{\Sigma_{in}}d\Omega_{3} (\cosh \tau)^{3}\tilde{\varphi} (\partial_{\tau}\varphi^{+}-\partial_{\tau}\varphi^{-})\bigg)
%\end{gathered}
%\end{equation}
%note we used $\varphi=\tilde{\varphi}$ at $\Sigma_{in}$. The integral over $\Omega_{3}$ in the linear term projects only the spatially homogeneous part of $\varphi$ to appear in the action. The contribution of $\varphi_{c}$ in this terms will give $I_{c}$ and the contribution from $\tilde{\varphi}$ comes purely from the $S^{4}$, e.g, the Euclidean section of the geometry. The boundary term is sometimes more conveniently evaluated by extending the boundary integral to all of $\Omega_{3}$, which is allowed since $\partial_{\tau}\varphi^{+}=\partial_{\tau}\varphi^{-}$ in $\Sigma_{out}$. This term will contain a contribution purely from $\tilde{\varphi}$ that will be the same as in the action \nref{ActFi} and an extra contribution from the derivative of $\varphi_{c}^{\pm}$, giving 
\begin{equation}
\begin{gathered}
\log p=\log p_{c}-\frac{8 \pi^{2}i \epsilon_{0}M_{pl}^{2}}{H_{r}^{2}}\bigg(2 c_{0}+\frac{1}{2}\sum_{l,m_{1},m_{2}}^{\infty} \frac{l(l+1)(l+2)}{1+\frac{l(l+2)}{\cosh^{2}\tau_{r}}}c_{l,m_{1},m_{2}}^{2}\bigg)
\end{gathered}
\end{equation}

Note that the scalar contribution for the probability density in $\tau_{r}=0$ agrees with the equation 23 discussed in \cite{Chen:2024rpx} for the Bunch-Davies vacuum. This should be the case, because the quantum field theory problem of computing the density matrix for the inflaton is the same in both vacuums. The difference is that the Hartle Hawking state is also taking into account the gravitational degrees of freedom. The final form of the action is thus, without any large $\tau$ approximation

\VI{It seems we got an interest in keeping finite $\tau$ effects sometimes so I thought I should include this equation, which has a role later in the fixed area problem. If we only want $\tau_{r}>>1$ I can just erase this}
\begin{equation}
\begin{gathered}
\label{OnshellactHH+Curvfinitetau}
\log p=S_{r}-\frac{8 \pi^{2}\epsilon_{0} M_{pl}^{2}}{H_{r}^{2}}\bigg(2 \ln \cosh \tau_{r}-\frac{2}{\cosh^{2}\tau_{r}}+2 c_{0}-2 \ln 2+\frac{17}{6}\\+\frac{1}{2}\sum_{l,m_{1},m_{2}}^{\infty} \frac{l(l+1)(l+2)}{1+\frac{l(l+2)}{\cosh^{2}\tau_{r}}}c_{l,m_{1},m_{2}}^{2}\bigg)
\end{gathered}
\end{equation}
where the coefficients $c_{l,m_{1},m_{2}}$ are determined by the system of equations
\begin{equation}
\begin{gathered}
\sum_{l,m_{1},m_{2}}c_{l,m_{1},m_{2}}Y_{l,m_{1},m_{2}}=\rho_{b}(\Omega_{3}) \text{, for } \vec{\Omega}_{3} \in \Sigma_{in}\\
\sum_{l,m_{1},m_{2}}^{\infty} \frac{l(l+1)(l+2)}{1+\frac{l(l+2)}{\cosh^{2}\tau_{r}}}c_{l,m_{1},m_{2}}Y_{l,m_{1},m_{2}}(\Omega_{3})=-2 \text{ for }\vec{\Omega}_{3} \in \Sigma_{out} \la{Eqns2Sol}
\end{gathered}
\end{equation}

However, while it is sensible to consider finite $\tau$ effects for the problem of the density matrix of $\varphi$ at $\tau=\tau_{r}$, we will here be mostly interested in studying the density matrix for the Weyl factor $\rho$ in a fixed $\phi$ surface, which is only related to the former problem when $\tau_{r}>>1$. From now on we therefore assume $\tau_{r}>>1$ unless otherwise stated. In this limit the action and boundary conditions are slightly simplified to
\begin{equation}
\begin{gathered}
\label{OnshellactHH}
\log p=S_{r}-\frac{8 \pi^{2}\epsilon_{0} M_{pl}^{2}}{H_{r}^{2}}\bigg(2 \tau_{r}+2 c_{0}-2 \ln 2+\frac{17}{6}+\frac{1}{2}\sum_{l,m_{1},m_{2}}^{\infty} l(l+1)(l+2)c_{l,m_{1},m_{2}}^{2}\bigg)
\end{gathered}
\end{equation}
with
\begin{equation}
\begin{gathered}
\sum_{l,m_{1},m_{2}}c_{l,m_{1},m_{2}}Y_{l,m_{1},m_{2}}=\rho_{b}(\Omega_{3}) \text{, for } \vec{\Omega}_{3} \in \Sigma_{in}\\
\sum_{l,m_{1},m_{2}}^{\infty} l(l+1)(l+2)c_{l,m_{1},m_{2}}Y_{l,m_{1},m_{2}}(\Omega_{3})=-2 \text{ for }\vec{\Omega}_{3} \in \Sigma_{out}
\end{gathered}
\end{equation}

In the following subsections we illustrate the method outlined above in a series of examples. 


==> MoreDiscBubble.tex <==
\VI{Here we want to discuss general aspects of these bubble solutions, maybe relations to eternal inflation and etc, but more importantly whether or not we can recover the result of usual slow-roll inflation by considering proper limits of the intervals in this bubble background.}

==> ReltoHH.tex <==
\VI{Here we want to explain how the prescription for the density matrix follows from the usual Hartle Hawking prescription, with proper gluings being performed. We should stress there is quite a lot of freedom on choosing the gluing slice. We should also stress that in principle not every density matrix could be obtained this way. That being said, we currently don't know any density matrix that does not come from applying a gluing procedure on a Hartle Hawking wavefunction} 

==> SK.tex <==
\VI{Here we want to explain general properties of Schwinger Keldysh contours that should be respected in the problems we consider. This is for example the fact the solutions on the bra and ket are related by complex conjugation and etc.}


\subsubsection{ \JM{ I propose to delete this whole subsection} \VI{I agree, with the current splitting we have now}}

It turns out to be convenient to write the solution as 
\be 
\varphi^\pm = \varphi^\pm_c + \tilde \varphi^\pm 
\ee 
where $\varphi_c$ is the same spatially homogenous solution we had in \nref{phic} and which obeyed the equation \nref{Eomvf}. This means that $\tilde \varphi^\pm$ obeys the homogeneous equation 
\be \la{Eomvft}
\nabla^2 \tilde \varphi = 0 
\ee 
For the diagonal case, this means that the boundary conditions \nref{EqnsTo} become
\bea
& ~& \tilde \varphi_+ = \tilde \varphi^- =    \rho(\Omega)   ~,~~~~~~~~~~~~~~~~~~~~~~~~~~~~{\rm for } ~~~~~~\tau = \tau_r ~,~~~~\vec \Omega \in \Sigma_{\pm \rm in}
\cr 
&~& \tilde \varphi_+ = \tilde \varphi_- ~,~~~~~~~i \cosh^2 \tau_r ( \partial_\tau \tilde \varphi_+ - \partial_\tau \tilde \varphi_- ) = 4   ~,~~~~~  
{\rm for }~~~~~~~~~\tau = \tau_r ~,~~~~\vec \Omega \in \Sigma_{\rm out} \la{EqnsTo2}
\eea 
where the 4 in the right hand side comes from the time derivatives of the solutions $\varphi_c^\pm$ after using \nref{DervFc}. 

We see that the problem is somewhat similar to the one for purely de-Sitter. It is not identical because in the case of de-Sitter we did not have the 4 in the right hand side of \nref{EqnsTo2}. 

We will discuss below how to find a solution of the equations \nref{EqnsTo}. We will now discuss how to evaluate the action.  

For the diagonal components the two surfaces $\Sigma_{\pm \rm in}$ coincide. 
In principle, we are supposed to evaluate the action along the surface with $\varphi =0$, which has a geometry given by the function $\rho$ as in \nref{3Geom} \nref{SliTau}. However, as we discussed in section \ref{superhorizon}, we can evaluate the action on a different slice, as long as we are at large $\tau$ (superhorizon distances) and we take into account the leading evolution of the fields into the new slice. 
This means that we can evaluate the action on a constant $\tau=\tau_r$ slice, where the scalar field takes the value \nref{varphiLa} with $f=\rho$. 
The gravity part of the action, the first line in \nref{AcSca} gives just the de-Sitter entropy as before. 
The second line in \nref{AcSca} involves  
\be \la{FinAcvf}
\int_{\cal M } [ \half (\nabla \varphi)^2 + 3 \varphi] = \int_{\Sigma_{\rm in}} \half \varphi \partial_n \varphi + { 3 \over 2 } \int_{\cal M } \varphi 
%\int_{\cal M}[  \half (\nabla \varphi_c)^2 + 3 \varphi_c ]  
%+\int_{\Sigma_{\rm in}} \tilde \varphi \partial_n \varphi_c
%+ \half \int_{\cal M} 3 \tilde \varphi + \int_{\Sigma_{\rm in}} \half \tilde \varphi \partial_n   \varphi 
\ee 
This identity is valid both form $\varphi$ or for $\varphi_c$. When we apply in the later case, it tells us that the bulk integral of $\varphi_c$ gives us the same as in \nref{Acco} or \nref{AcLat} since $\varphi_c$ vanishes at the boundary. Then we can write
\be \la{FinAcvf2}
\int_{\cal M } [ \half (\nabla \varphi)^2 + 3 \varphi] = \hat I_c + \int_{\Sigma_{\rm in}} \half \tilde \varphi \partial_n \varphi + { 1 \over 2 } \int_{\cal M } 3 \tilde \varphi ~,~~~~~~~~~\hat I_c \equiv \half \int_{\cal M } 3 \varphi_c
\ee 
The first integral can be extended from $\Sigma_{\rm in}$ to the full spatial slice  because $\partial_t \varphi^+ = \partial_t \varphi^-$ on $\Sigma_{\rm out}$. Finally, we write the $3 = \nabla^2 \varphi_c$ in the last term, and we integrate by parts. 
When we do so, we will pick up terms on the whole spatial slice, because it is for  only the full field $\varphi$ that $\Sigma_{\rm out}$ is not a boundary. Then we get 
\be 
\log p =  \log p_{c} + { 2 \epsilon_r M_{pl}^2 \over H_r^2 } 
  \int_{S^3} d\Omega_3 \left[ \half \tilde \varphi   \cosh^3 \tau_r (i\partial_t \tilde \varphi^+ - i\partial_t \tilde \varphi^-)  -  4 \tilde \varphi  \right] \la{ActForF}
\ee 
  where the last factor of 4 arose by using  \nref{DervFc} and the integral is over a unit radius $S^3$.  And $\log p_c$ is given in \ref{Acco}.
 
  


%Then we write $\varphi = \varphi_c + \tilde \varphi $ where $\tilde \varphi$ obeys the equation $\nabla \tilde \varphi^2 =0$, so that it is similar to the problem of the scalar field in de-Sitter that we considered above. It is not completely identical because now the boundary conditions have the form 
%\bea 
%& ~& \tilde \varphi^+ = \tilde \varphi^- = \rho ~,~~~~~~ {\rm for } ~~~~\tau= \tau_r ~,~~~~\vec \Omega \in \Sigma_{\pm in}
%\cr 
%& ~& \tilde \varphi^+ = \tilde \varphi^- ~,~~~~~~ \partial_\tau \tilde \varphi^+ - \partial_\tau \tilde \varphi^- = - ( \partial_\tau \varphi_c^+ - \partial_\tau \varphi_c^-)  ~,~~~~~~ {\rm for } ~~~~\tau= \tau_r ~,~~~~\vec \Omega \in \Sigma_{\pm in}
%\eea

%We want to consider the problem of what is the probability measure of the geometry of the reheating surface at the end of inflation. To make the calculation simpler, we rely on the saddle point approximation, and we solve for the classical solution perturbatively in the slow-roll parameters. To understand this point, take the extreme case of slow-roll where $V(\phi)=V_{0}$ is a constant. In that case the inflaton does not roll and the equations of motion have an exact de Sitter solution, with
%\begin{equation}
%\begin{gathered}
%ds^{2}=\frac{1}{H_{0}^{2}}(-d\tau^{2}+\cosh^{2}\tau\, d\Omega_{3}^{2}) \text{, and } \phi=\phi_{0}\text{, with }H_{0}^{2}=\frac{V(\phi_{0})}{3 M_{pl}^{2}}
%\end{gathered}
%\end{equation}

%Then, if we for example fix the universe at the reheating surface $\Sigma$ to be $S^{3}$ with radius $a_{r}$ and the inflaton to be $\phi_{0}=\phi_{r}$, it must be that the saddle is the de Sitter solution with radius fixed by $\phi_{0}=\phi_{r}$, and $\Sigma$ is a fixed $\tau$ surface with $\tau$ fixed by the ratio of $a_{r}$ to the de Sitter radius. In general, $\Sigma$ will be a codimension one surface in de Sitter such that the boundary conditions for its intrinsic metric are respected. Our perspective is that the actual saddle can be found perturbatively around this zeroth order one, e.g, one can expand the actual solution as
%\begin{equation}
%\phi=\phi_{0}+\delta \phi \text{, } \tilde{g}_{a b}=g_{a b}+\delta g_{a b}
%\end{equation}
%with $g_{a b}$ the metric of pure de Sitter with radius $H_{r}^{-1}$, and $\delta \phi$ and $\delta g_{a b}$ perturbative corrections. Since the fields $\phi_{0}$ and $g_{a b}$ already respected the boundary conditions at $\Sigma$, we must also impose that both the perturbation in the field and the metric vanish there, e.g
%\begin{equation}
%\delta \phi|_{\Sigma}=\delta h_{a b}|_{\Sigma}=0
%\end{equation}
%with $h_{a b}$ the induced metric in $\Sigma$. The perturbative expansion we do is on in $V'(\phi_{0})$, neglecting corrections due to $V_{0}''$, $V_{0}'''$ and higher order derivatives. \YC{(Should higher derivatives terms be the order of $\epsilon_0^\#$ in the standard slow roll inflation? We ignore them because we only keep to $\epsilon_0$.)}\VI{I am not sure, I think at order $\epsilon_{0}$ there could be terms coming from $V''$ as well. } \YC{(In this approximation, probably no, right? $V\sim V_0 + V' \delta\phi + V'' \delta\phi^2$, the third term is $\epsilon_0^2$ order)}\VI{I do not know if there could be problems somewhere else, I just posed the problem like I think Juan mentioned it first. Maybe what you said is also correct, but we need to discuss more to be sure.} From the scalar equation of motion one can see that $\delta \phi \sim V'$, and the backreaction of the metric will be due to the shift in the stress tensor. The shift in the stress tensor will contain terms such as $V' \delta \phi\sim V'^{2}$ and $(\partial \phi)^{2} \sim V'^{2}$. Therefore, the metric perturbation will be of order $\delta g_{ab} \sim V'^{2}$ \footnote{There could in principle be metric perturbation at order $V'$, they would be homogeneous solutions of linearized gravity around the zeroth order background. However, imposing that $\delta h_{a b(1)}=0$ in the boundary fixes the whole function to be zero}. The dimensionless pertubative parameter will be
%\begin{equation}
%\epsilon_{0}=\frac{1}{2}M_{pl}^{2}\frac{V'(\phi_{0})^{2}}{V(\phi_{0})^{2}}
%\end{equation}
%with $\phi_{0}$ the relevant value of $\phi$ we expand around. The perturbative expansion will then therefore be of form
%\begin{equation}
%\begin{gathered}
%\delta \phi=M_{pl}^{\frac{D-2}{2}}\big[\sqrt{2\epsilon_{0}}\varphi_{1}+(\sqrt{2\epsilon_{0}})^{2}\varphi_{2}+...\\
%\delta g_{a b}=H_{0}^{-2}\big[(\sqrt{2\epsilon_{0}})^{2}\delta g_{a b (2)}+....
%\end{gathered}
%\end{equation}
%which implies that the perturbed action will be at least of order $\epsilon_{0}$. Therefore, to obtain the leading order action we need to vary the action to first order in the metric, and in principle to second order in $\phi$, keeping only terms of order $\epsilon_{0}$. The change in the action at the linear order in the metric, but exact in $\phi$, will be
%\begin{equation}
%\begin{gathered}
%\frac{M_{pl}^{2}}{2}\bigg(\int_{\mathcal{M}} d^{4}x\, \sqrt{-g}\bigg[-\bigg(R^{a b}-\frac{1}{2}g^{a b}R-T_{a b}(g_{a b},\phi_{0}+\delta \phi)\bigg)\delta g_{a b}
%\\-\frac{M_{pl}^{2}}{2}\int_{\partial \mathcal{M}}d^{3}x\, \sqrt{h}(h^{a b}K-K^{a b})\delta h_{a b}
%\end{gathered}
%\end{equation}
%and since Einstein equation is zero at zeroth order in $\epsilon_{0}$, $\delta g_{a b}$ times Einstein equation will be at order higher than $\epsilon_{0}$, thus we can ignore the bulk term O($\epsilon_{0}$). The boundary term is also zero, since the only boundary of the manifold are those of the bra and the ket, where $\delta h_{a b}=0$ by consistency of the perturbative expansion. The action of the scalar at this order therefore comes simple from the slope term $V'_{r}\delta \phi$ and the kinect term $g^{a b}\partial_{a}\delta \phi \partial_{b}\delta \phi$. Putting everything together we find that the action at order $\epsilon_{0}$ is 



%\begin{equation}
%\begin{gathered}
%\delta I_{2}=\frac{2 \epsilon_{0}M_{pl}^{2}}{H_{0}^{2}}\int_{\mathcal{M}} d^{4}x\, \sqrt{-g} \bigg(-\frac{1}{2}g^{a b}\partial_{a}\varphi_{1}^{\pm} \partial_{b}\varphi_{1}^{\pm}-3\varphi_{1}^{\pm}\bigg)
%\end{gathered}
%\end{equation}
%where the integral is over $\mathcal{M}=dS_{4}$, e.g, a unit radius de Sitter geometry that has the proper analytic continuation giving the no-boundary geometry for the problem. The on-shell action respecting the boundary conditions is greatly simplified, the equation of motion for $\varphi_{1}$ is
%\begin{equation}
%\label{varphieq}
%-\nabla_{1}^{2}\varphi_{1}+3=0
%\end{equation}
%with $\nabla_{1}^{2}$ the laplacian on $dS_{4}$. Using the equations of motion and integration by parts, and that $\varphi_{1}|_{\Sigma_{in}}=0$, one finds that the on-shell action at this order is
%\begin{equation}
%\begin{gathered}
%\label{OnshellactHH}
%\delta I_{2}=-\frac{3 \epsilon_{0}M_{pl}^{2}}{H_{0}^{2}}\int_{\mathcal{M}} d^{4}x\, \sqrt{-g}\varphi_{1}
%\end{gathered}
%\end{equation}

%To avoid cumbersome notation we refer to $\varphi_{1}$ as $\varphi$ from now on.


